Localizing Router Configuration Errors Using Minimal Correction Sets

Router configuration errors are unfortunately common and difficult to localize using current network verifiers. We introduce a novel configuration error localizer (CEL) that precisely identifies which configuration segments contribute to the violation of forwarding requirements. In particular, CEL generates a system of satisfiability modulo theories (SMT) constraints-which encode a network's configurations, control logic, and forwarding requirements-and uses a domain-specific minimal correction set (MCS) enumeration algorithm to identify problematic configuration segments. CEL efficiently locates several configuration errors in real university networks and identifies all routing-related and at least half of all ACL-related errors we introduce.

==> algorithms/encoding_talk.tex <==
\begin{figure}[t]
    \begin{subfigure}{1\columnwidth}
    \begin{algorithm}[H]
    \small
    \If(\tcp*[h]{Accept all exported}){$\outgoing{OSPF}{\routerOne}{\routerThree}.\valid$}{
        $\incoming{OSPF}{\routerThree}{\routerOne}.\valid = \true$\;
        $\incoming{OSPF}{\routerThree}{\routerOne}.\prefix = \outgoing{OSPF}{\routerOne}{\routerThree}.\prefix$\;
        $\incoming{OSPF}{\routerThree}{\routerOne}.\cost = \outgoing{OSPF}{\routerOne}{\routerThree}.\cost$\;
        }
    \lElse{$\incoming{OSPF}{\routerThree}{\routerOne}.\valid = \false$ \tcp*[h]{None imported}}
    \end{algorithm}
    \caption{\routerThree import from \routerOne}
    \label{fig:encoding_r3_import}
    \end{subfigure}
    
    \begin{subfigure}{1\columnwidth}
    \begin{algorithm}[H]
    \small
    \setstretch{1.2}
    \If(\tcp*[h]{Originate \subnetT}){$\destination \in
    10.0.20.0/24$\hspace{1em}\ }{
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\prefix = 10.0.20.0/24$\;
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\cost = 1$\;
    }
    \ElseIf(\tcp*[h]{Forward shortest}){$\best{OSPF}{\routerThree}.\valid$}{
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\valid = \true$\;
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\prefix = \best{OSPF}{\routerThree}.\prefix$\;
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\cost = \best{OSPF}{\routerThree}.\cost + 1$\;
    }
    \lElse{$\outgoing{OSPF}{\routerThree}{\routerOne}.\valid = \false$ \tcp*[h]{None exported}}
    \end{algorithm}
    \caption{\routerThree export to \routerOne}
    \label{fig:encoding_r3_export}
    \end{subfigure}
    
    \begin{subfigure}{1\columnwidth}
    \begin{algorithm}[H]
    \small
    \setstretch{1.2}
    $\forward{}{\routerOne}{\routerThree} \iff \best{Overall}{\routerOne} = \incoming{OSPF}{\routerOne}{\routerThree}$\;
    \Indp
    $\land\ \neg(\destination \in 10.0.20.0/24)$ \tcp*[h]{ACL}
    \end{algorithm}
    \caption{\routerOne forward to \routerThree}
    \label{fig:encoding_r1_forward}
    \end{subfigure}

    \begin{subfigure}{1\columnwidth}
    \begin{algorithm}[H]
    \small
%    \If{\configOspfAdjacency{\routerThree}{\routerOne}}{
    \If{$\destination \in \configOspfOriginate{\routerThree}{10.0.20.0/24}$}{
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\prefix =
        \configOspfOriginate{\routerThree}{10.0.20.0/24}$\;
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\cost = \configOspfCost{\routerThree}{\routerOne}$\;
    }
    \ElseIf{$\best{OSPF}{\routerThree}.\valid \land \configOspfFilterDefault{\routerThree}$}{
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\valid = \true$\;
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\prefix = \best{OSPF}{\routerThree}.\prefix$\;
        $\outgoing{OSPF}{\routerThree}{\routerOne}.\cost = \best{OSPF}{\routerThree}.\cost + \configOspfCost{\routerThree}{\routerOne}$\;
    }
    \lElse{$\outgoing{OSPF}{\routerThree}{\routerOne}.\valid = \false$}
%    }
%    \lElse{$\outgoing{OSPF}{\routerThree}{\routerOne}.\valid = \false$}
    \end{algorithm}
    \caption{\routerThree export to \routerOne}
    \label{fig:encoding_symbolic_r3_export}
    \end{subfigure}

    \begin{subfigure}{1\columnwidth}
    \begin{algorithm}[H]
    \small
    $\forward{}{\routerOne}{\routerThree} \iff \best{Overall}{\routerOne} = \incoming{OSPF}{\routerOne}{\routerThree}$\;
    \Indp
    $\land\ \configAcl{\coreOneRouter}{filterT}$
    \end{algorithm}
    \caption{\routerOne forward to \routerThree}
    \label{fig:encoding_symbolic_r1_forward}
    \end{subfigure}
    
    \begin{subfigure}{1\columnwidth}
    \begin{algorithm}[H]
    \small
    $\configOspfOriginate{\routerThree}{10.0.20.0/24} = 10.0.20.0/24$\;
    $\configOspfCost{\routerThree}{\routerOne} = 1$\;
    $\configAcl{\routerThree}{filterT} = \neg (\destination \in 10.0.20.0/24)$\;
    $\configOspfAdjacency{\routerThree}{\routerOne} = \true$\;
    $\configOspfFilterDefault{\routerThree} = \true$\;
    $\configOspfAdjacency{\routerTwo}{\routerOne} = \false$\;
    \end{algorithm}
    \caption{Configuration}
    \label{fig:encoding_symbolic_config_talk}
    \end{subfigure}
    
    \begin{subfigure}{1\columnwidth}
    \begin{algorithm}[H]
    \small
    \If{\configOspfAdjacency{\routerTwo}{\routerOne}}{
        $\ldots$
    }
    \lElse{$\outgoing{OSPF}{\routerTwo}{\routerOne}.\valid = \false$}
    \end{algorithm}
    \caption{\routerTwo export to \routerOne}
    \label{fig:encoding_symbolic_r2_export}
    \end{subfigure}


    
    
    \caption{Constraints encoding part of the behavior of the example network
    in \figref{fig:challenges_example3}}
    \label{fig:encoding_talk}
\end{figure}


==> tables/campus_networks.tex <==
\begin{table}
\small
\begin{tabular}{cccc}
Network & Users & Routers & Protocols \\
\hline
\colgate & $\approx$4k & 3 & iBGP \\
\uwmadison& $\approx$65k & 11 & OSPF (iBGP excluded)\\
\northwestern & $\approx$30k & 28 & OSPF (iBGP excluded) \\
\end{tabular}
\caption{Campus networks}
\label{tbl:campus_networks}
\end{table}
